Securing Deep Learning Hardware: A Survey of Side-Channel Vulnerabilities and Countermeasures

As deep learning models are increasingly deployed in critical sectors such as healthcare, finance, and security, ensuring their protection against emerging threats has become crucial. Among these threats, side-channel attacks (SCAs) represent a particular challenge since they can extract sensitive information such as model architectures, parameters, and even user inputs without requiring direct access to the model. By leveraging the physical and micro-architectural properties of the hardware, attackers can compromise systems. This survey begins by classifying leakage sources and attacker objectives, then analyzes representative studies that demonstrate practical side-channel exploits against deep-learning hardware. It also reviews existing defenses aimed at mitigating these vulnerabilities and concludes by outlining key open research challenges and potential future directions.

==> Style/Theorem-Styles.tex <==
\RequirePackage{amsthm}%
\def\th@plain{%
\thm@preskip\parskip
\thm@postskip\z@
\itshape % body font
}
\def\th@definition{%
\thm@preskip\parskip
\thm@postskip\z@
\normalfont % body font
}
\def\th@remark{%
\thm@headfont{\itshape}%
\normalfont % body font
\thm@preskip\parskip \divide\thm@preskip\tw@
\thm@postskip\z@
}

%\newenvironment{pf}%
%  {\par\addvspace{\@bls \@plus 0.5\@bls \@minus 0.1\@bls}\noindent
%   {\bfseries\Elproofname}\enspace\ignorespaces}%
%  {\par\addvspace{\@bls \@plus 0.5\@bls \@minus 0.1\@bls}}
%\def\Elproofname{PROOF.}
%\@namedef{pf*}#1{\par\begingroup\def\Elproofname{#1}\pf\endgroup\ignorespaces}
%\expandafter\let\csname endpf*\endcsname=\endpf


\newtheoremstyle{XYZ}% name
{3pt}% Space above
{3pt}% Space below
{}% Body font
{}% Indent amount
{\bfseries}% Theorem head font
{}% Punctuation after theorem head
{.5em}% Space after theorem head
{\bfseries{#1 #2\if#3\else~(#3)\fi.}}% Theorem head spec (can be left empty, meaning `normal')



\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{claim}{Claim}
\newtheorem{axiom}{Axiom}
\newtheorem{conjecture}{Conjecture}
\newtheorem{fact}{Fact}
\newtheorem{hypothesis}{Hypothesis}
\newtheorem{assumtion}{Assumption}
\newtheorem{criterion}{Criterion}
\theoremstyle{XYZ}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{remark}{Remark}
\newtheorem{notation}{Notation}
\newtheorem{problem}{Problem}
\newtheorem{principle}{Principle} 
